Using did_multiplegt_dyn to Estimate Event-Study Effects in Complex Designs: Overview, and Four Examples Based on Real Datasets

The command did_multiplegt_dyn can be used to estimate event-study effects in complex designs with a potentially non-binary and/or non-absorbing treatment. This paper starts by providing an overview of the estimators computed by the command. Then, simulations based on three real datasets are used to demonstrate the estimators' properties. Finally, the command is used on four real datasets to estimate event-study effects in complex designs. The first example has a binary treatment that can turn on an off. The second example has a continuous absorbing treatment. The third example has a discrete multivalued treatment that can increase or decrease multiple times over time. The fourth example has two, binary and absorbing treatments, where the second treatment always happens after the first.

==> Table_app.tex <==
\begin{center}
\begin{table}[h!]
\caption{Simulation Results \st{did\_multiplegt\_dyn}, Reduced Sample}
\label{tbl:sim_app}
\scriptsize
\begin{tabular}{lcccccccc}
\midrule[2pt]
\textbf{Design} & \textbf{Effect\_1} & \textbf{Effect\_2} & \textbf{Effec\_3} & \textbf{Avg\_Effect} & \textbf{Placebo\_1} & \textbf{Placebo\_2} & \textbf{Placebo\_3} & F\_test\_placebo \\ \midrule
\midrule
N=100 & 0.9585 & 0.953 & 0.9465 & 0.9365 & 0.953 & 0.9455 & 0.942 & 0.0635  \\
N=50 & 0.938 & 0.953 & 0.949 & 0.9475 & 0.934 & 0.9345 & 0.936 & 0.089  \\
N=30 & 0.9325 & 0.931 & 0.934 & 0.934 & 0.943 & 0.94 & 0.934 & 0.1155  \\
N=20 & 0.918 & 0.927 & 0.9385 & 0.9355 & 0.914 & 0.939 & 0.9155 & 0.1715  \\
\midrule[2pt]
\end{tabular}
    \begin{minipage}\textwidth 
 \footnotesize{\textit{Notes:} Table \ref{tbl:sim_app} shows the coverage rates and p-values from the simulations described at the beginning of section \ref{sec:simulations}, conducted on the dataset from \cite{vella1998whose}. They resemble the baseline case from Table \ref{tbl:sim_main} with a reduced number of groups (N). All simulations were repeated 2000 times.}
    \end{minipage}
\end{table}

% & F\_test\_effect 
% & 0.0565
% & 0.065
% & 0.081
% & 0.123

\end{center}

==> table.tex <==
\begin{center}
\begin{table}[h!]
\scriptsize
\begin{tabular}{ccccccccc}
\midrule[2pt]
\textbf{Effect\_1} & \textbf{Effect\_2} & \textbf{Effec\_3} & \textbf{Avg\_Effect} & \textbf{Placebo\_1} & \textbf{Placebo\_2} & \textbf{Placebo\_3} & F\_test\_placebo & F\_test\_effect \\ \midrule
\midrule
\multicolumn{9}{c}{\footnotesize \textbf{Panel A: }}\\\midrule
0.9435 & 0.9505 & 0.9515 & 0.946 & 0.949 & 0.9425 & 0.946 & 0.0615 & 0.05 \\
0.9435 & 0.9505 & 0.9515 & 0.946 & 0.949 & 0.9425 & 0.946 & 0.0615 & 0 \\
0.952 & 0.9525 & 0.9465 & 0.946 & 0.951 & 0.9485 & 0.947 &  &  \\
0.9475 & 0.9465 & 0.9505 & 0.9425 & 0.9385 & 0.9415 & 0.939 &  &  \\
0.9555 & 0.951 & 0.9255 & 0.923 & 0.9535 & 0.9575 & 0.9495 &  &  \\
0.9435 & 0.9505 & 0.9515 & 0.946 & 0.949 & 0.9425 & 0.946 & 0.0615 & 0 \\
0.946 & 0.9495 & 0.952 & 0.9465 & 0.951 & 0.9435 & 0.947 & 0.0565 & 0 \\\midrule
\multicolumn{9}{c}{\footnotesize \textbf{Panel B: }}\\\midrule
0.941 & 0.939 & 0.9395 & 0 & 0.945 & 0.9455 &  & 0.0525 & 0 \\
0.9465 & 0.9505 & 0.949 & 0.9495 & 0.9495 & 0.9385 & 0.9415 & 0.066 & 0 \\
0.9495 & 0.9455 & 0.941 & 0.9415 & 0.9435 & 0.94 & 0.9445 & 0.0725 & 0 \\
0.947 & 0.946 & 0.9445 & 0.9465 & 0.945 & 0.9435 & 0.935 & 0.0785 & 0 \\
0.95 & 0.9475 & 0.947 & 0.9485 & 0.9485 & 0.9465 & 0.9435 & 0.068 & 0 \\
0.949 & 1 & 0.9995 & 0.998 & 0.9385 & 0.958 & 0.9555 & 0.045 & 0 \\
\midrule
\multicolumn{9}{c}{\footnotesize \textbf{Panel C: }}\\\midrule
0.949 & 0.9465 & 0.9645 & 0.9525 & 0.9385 & 0.958 & 0.9555 & 0.045 & 0 \\
0.9585 & 0.953 & 0.9465 & 0.9365 & 0.953 & 0.9455 & 0.942 & 0.0635 & 0.0565 \\
0.938 & 0.953 & 0.949 & 0.9475 & 0.934 & 0.9345 & 0.936 & 0.089 & 0.065 \\
0.9325 & 0.931 & 0.934 & 0.934 & 0.943 & 0.94 & 0.934 & 0.1155 & 0.081 \\
0.918 & 0.927 & 0.9385 & 0.9355 & 0.914 & 0.939 & 0.9155 & 0.1715 & 0.123 \\
0.97 & 0.982 & 0.9865 & 0.983 & 0.9715 & 0.954 & 0.9635 & 0.037 & 0 \\
\midrule[2pt]
\end{tabular}
\end{table}
\end{center}
